A first application of the Alcock-Paczynski test to stacked cosmic voids

We report on the first application of the Alcock-Paczynski test to stacked voids in spectroscopic galaxy redshift surveys.We use voids from the Sutter et al. (2012) void catalog, which was derived from the Sloan Digital Sky Survey Data Release 7 main sample and luminous red galaxy catalogs. The construction of that void catalog removes potential shape measurement bias by using a modified version of the ZOBOV algorithm and by removing voids near survey boundaries and masks. We apply the shape-fitting procedure presented in Lavaux & Wandelt (2012) to ten void stacks out to redshift z=0.36. Combining these measurements, we determine the mean cosmologically induced "stretch" of voids in three redshift bins, with 1-sigma errors of 5-15%. The mean stretch is consistent with unity, providing no indication of a distortion induced by peculiar velocities. While the statistical errors are too large to detect the Alcock-Paczynski effect over our limited redshift range, this proof-of-concept analysis defines procedures that can be applied to larger spectroscopic galaxy surveys at higher redshifts to constrain dark energy using the expected statistical isotropy of structures that are minimally affected by uncertainties in galaxy velocity bias.

==> tab_samples.tex <==
dim1 & NYU VAGC & -18.9 & 0.0 & 0.05 & 63639 &  3\\ 
dim2 & NYU VAGC & -20.4 & 0.05 & 0.1 & 156266 &  5\\ 
bright1 & NYU VAGC & -21.35 & 0.1 & 0.15 & 113713 &  8\\ 
bright2 & NYU VAGC & -22.05 & 0.15 & 0.2 & 43340 & 13\\ 
lrgdim & LRGs & -21.2 & 0.16 & 0.36 & 67567 & 24\\ 
lrgbright & LRGs & -21.8 & 0.36 & 0.44 & 15212 & 38\\ 

